EVISKILL: Grounding Skill Evolution in Replayable Evidence

Continual skill evolution enables LLM agents to accumulate and refine reusable procedural knowledge from interaction experience without updating model parameters. Its effectiveness depends on determining not only what to change, but also why a change is justified and when it should become persistent guidance. However, existing experience-driven methods can lose the behavioral evidence and task contexts supporting edits. Moreover, a global validation outcome provides an incomplete judgment of its constituent changes: locally supported corrections may be discarded with a rejected revision, while evidence may require further experience to inform useful updates. To this end, we introduce EVISKILL, an evidence-driven framework that organizes execution observations into Replayable Evidence Cards and synthesizes edits with explicit links to their supporting contexts. Targeted replay verifies these edits through re-execution and provides feedback for correction. Across epochs, EVISKILL preserves evidence and provisionally retains supported edits for further refinement, while global validation governs their incorporation into the final skill. Experiments on three interactive benchmarks across six LLM backbones demonstrate the effectiveness of this approach.

==> experiment/ablation.tex <==
% Requires: \usepackage{booktabs,tabularx,array}
\begin{table}[t]
\caption{Protocol-matched component ablations. Values are hard-success
accuracy (\%); parentheses give the absolute percentage-point change
from Full, so a positive value means that the ablated variant scores
higher.}
\label{tab:ablation}
\centering
\fontsize{6.2}{7.0}\selectfont
\setlength{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabularx}{\columnwidth}{@{}
>{\hsize=1.15\hsize\raggedright\arraybackslash}X
>{\hsize=1.15\hsize\raggedright\arraybackslash}X
>{\hsize=.80\hsize\raggedleft\arraybackslash}X
>{\hsize=.95\hsize\raggedleft\arraybackslash}X
>{\hsize=.95\hsize\raggedleft\arraybackslash}X@{}}
\toprule
Dataset & Model & Full & w/o Replay & w/o Cross-Epoch \\
\midrule
ALFWorld & GPT-5.5
& 96.27 & 93.28 ($-$2.99) & 94.78 ($-$1.49) \\

ALFWorld & GPT-5.4
& 95.52 & 94.78 ($-$0.74) & 94.03 ($-$1.49) \\

ALFWorld & GPT-5.4-mini
& 91.79 & 88.06 ($-$3.73) & 90.30 ($-$1.49) \\

ALFWorld & Qwen-3.5-4b
& 85.07 & 82.09 ($-$2.98) & 80.60 ($-$4.47) \\

ALFWorld & Qwen-3.5-9b
& 91.04 & 88.06 ($-$2.98) & 86.57 ($-$4.47) \\

ALFWorld & Qwen-3.5-35b
& 88.06 & 87.31 ($-$0.75) & 86.57 ($-$1.49) \\

\midrule
AppWorld & GPT-5.5
& 94.64 & 88.69 ($-$5.95) & 86.31 ($-$8.33) \\

AppWorld & GPT-5.4
& 90.48 & 85.12 ($-$5.36) & 89.29 ($-$1.19) \\

AppWorld & GPT-5.4-mini
& 83.93 & 81.55 ($-$2.38) & 80.95 ($-$2.98) \\

AppWorld & Qwen-3.5-4b
& 32.14 & 25.60 ($-$6.54) & 29.17 ($-$2.97) \\

AppWorld & Qwen-3.5-9b
& 43.45 & 44.05 (+0.60) & 41.67 ($-$1.78) \\

AppWorld & Qwen-3.5-35b
& 63.10 & 59.52 ($-$3.58) & 62.50 ($-$0.60) \\

\midrule
ScienceWorld & GPT-5.5
& 83.41 & 81.99 ($-$1.42) & 83.89 (+0.48) \\

ScienceWorld & GPT-5.4
& 76.78 & 74.88 ($-$1.90) & 71.09 ($-$5.69) \\

ScienceWorld & GPT-5.4-mini
& 67.78 & 62.56 ($-$5.22) & 69.67 (+1.89) \\

ScienceWorld & Qwen-3.5-4b
& 20.85 & 22.75 (+1.90) & 16.59 ($-$4.26) \\

ScienceWorld & Qwen-3.5-9b
& 37.91 & 36.02 ($-$1.89) & 37.91 (0.00) \\

ScienceWorld & Qwen-3.5-35b
& 40.76 & 39.34 ($-$1.42) & 40.28 ($-$0.48) \\

\midrule
Macro average & ---
& 71.28 & 68.65 ($-$2.63) & 69.01 ($-$2.27) \\
\bottomrule
\end{tabularx}
\end{table}

==> experiment/ablation_full.tex <==
% Requires: \usepackage{booktabs,tabularx,array}
\begin{table}[t]
\caption{Protocol-matched component ablations. Values are hard-success
accuracy (\%); parentheses give the absolute percentage-point change
from Full, so a positive value means that the ablated variant scores
higher.}
\label{tab:ablation}
\centering
\fontsize{6.2}{7.0}\selectfont
\setlength{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabularx}{\columnwidth}{@{}
>{\hsize=1.15\hsize\raggedright\arraybackslash}X
>{\hsize=1.15\hsize\raggedright\arraybackslash}X
>{\hsize=.80\hsize\raggedleft\arraybackslash}X
>{\hsize=.95\hsize\raggedleft\arraybackslash}X
>{\hsize=.95\hsize\raggedleft\arraybackslash}X@{}}
\toprule
Dataset & Model & Full & w/o Replay & w/o Cross-Epoch \\
\midrule
ALFWorld & GPT-5.5
& 96.27 & 93.28 ($-$2.99) & 94.78 ($-$1.49) \\

ALFWorld & GPT-5.4
& 95.52 & 94.78 ($-$0.74) & 95.52 (0.00) \\

ALFWorld & GPT-5.4-mini
& 91.79 & 91.79 (0.00) & 90.30 ($-$1.49) \\

ALFWorld & Qwen-3.5-4b
& 85.07 & 82.09 ($-$2.98) & 80.60 ($-$4.47) \\

ALFWorld & Qwen-3.5-9b
& 91.04 & 88.06 ($-$2.98) & 86.57 ($-$4.47) \\

ALFWorld & Qwen-3.5-35b
& 88.06 & 87.31 ($-$0.75) & 88.06 (0.00) \\

\midrule
AppWorld & GPT-5.5
& 94.64 & 88.69 ($-$5.95) & 86.31 ($-$8.33) \\

AppWorld & GPT-5.4
& 90.48 & 85.12 ($-$5.36) & 90.48 (0.00) \\

AppWorld & GPT-5.4-mini
& 83.93 & 81.55 ($-$2.38) & 83.93 (0.00) \\

AppWorld & Qwen-3.5-4b
& 32.14 & 25.60 ($-$6.54) & 29.17 ($-$2.97) \\

AppWorld & Qwen-3.5-9b
& 43.45 & 49.40 (+5.95) & 41.67 ($-$1.78) \\

AppWorld & Qwen-3.5-35b
& 63.10 & 59.52 ($-$3.58) & 62.50 ($-$0.60) \\

\midrule
ScienceWorld & GPT-5.5
& 83.41 & 81.99 ($-$1.42) & 88.63 (+5.22) \\

ScienceWorld & GPT-5.4
& 76.78 & 74.88 ($-$1.90) & 71.09 ($-$5.69) \\

ScienceWorld & GPT-5.4-mini
& 67.78 & 62.56 ($-$5.22) & 69.67 (+1.89) \\

ScienceWorld & Qwen-3.5-4b
& 20.85 & 26.07 (+5.22) & 16.59 ($-$4.26) \\

ScienceWorld & Qwen-3.5-9b
& 37.91 & 43.13 (+5.22) & 37.91 (0.00) \\

ScienceWorld & Qwen-3.5-35b
& 40.76 & 45.50 (+4.74) & 51.18 (+10.42) \\

\midrule
Macro average & ---
& 71.28 & 70.07 ($-$1.20) & 70.52 ($-$0.75) \\
\bottomrule
\end{tabularx}
\end{table}

==> experiment/cross_epoch_retention.tex <==
% Cross-epoch Provisional-edit retention and promotion.
\paragraph{Post-rejection edit pipeline and source-edit fate.}

We audit the post-validation-rejection pathway in the frozen 16-run Full
manifest.  Figure~\ref{fig:cross_epoch_retention} follows the pathway at two
levels: panel~(a) reports aggregate event counts from candidate generation
through replay allocation, replay acceptance, and Provisional-ledger
representation, while panel~(b) follows the terminal fate of the replay-
accepted source-edit cohort.

Across the three datasets, 155 candidate edits are generated after rejection.
Of these, 128 (82.6\%) are allocated to post-rejection replay, 97 (75.8\% of
allocated edits) are accepted, and 96 (61.9\% of candidates) are represented
in the Provisional ledger.  Panel~(a) shows the corresponding dataset curves
and the pooled overall trajectory; the stages are aggregate counts and are not
intended as item-level matching across stages.

Conditioning on the 97 replay-accepted source-edit events, panel~(b) shows
that 45 (46.4\%) are promoted after one epoch and 10 (10.3\%) after two
epochs.  Another 41 (42.3\%) remain active at the four-epoch horizon and are
therefore right-censored, while one event (1.0\%) fails reconciliation.  Thus,
55 of 97 accepted events are later promoted and 96 of 97 are represented in
the ledger.  This is a lifecycle audit of persistence and promotion, rather
than a causal comparison of validation accuracy.

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{Figure/cross_epoch_retention_lifecycle.pdf}
  \caption{Cross-epoch Provisional-edit retention and promotion.  Panel~(a)
  tracks post-rejection candidate edits through replay allocation, replay
  acceptance, and Provisional-ledger representation; colored curves show the
  three datasets and the dashed curve shows their pooled total.  Panel~(b)
  partitions the 97 replay-accepted source-edit events by terminal fate.
  ``Active at E4'' is right-censored, and ``Failure'' denotes reconciliation
  failure.  Percentages in panel~(b) are within-row shares from the frozen
  16-run formal manifest.}
  \label{fig:cross_epoch_retention}
\end{figure*}


==> experiment/evidence_lifecycle.tex <==
% Cross-epoch lifecycle analysis of Replayable Evidence Cards.
\paragraph{Evidence lifecycle and reuse.}

We track each unique $(\mathrm{run\_id},\mathrm{evidence\_id})$ across the 64
skill-evolution epochs.  Figure~\ref{fig:evidence_lifecycle} gives two
complementary views: panel (a) reports the per-epoch resolution of the input
pool into archived, stale, and active-after-epoch Cards, while panel (b)
reports the distribution of how many distinct epochs select each Card through
an Evidence Window.  Together they show both terminal resolution and the
reusable cross-epoch subset of the Evidence Pool.

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{Figure/evidence_lifecycle.pdf}
  \caption{Cross-epoch Evidence lifecycle over four skill-evolution epochs.
  (a) Per-epoch resolution of the input pool into \texttt{archived},
  \texttt{stale}, and \texttt{active after epoch}.  (b) Dataset-level
  distribution of the number of distinct epochs in which a Card is selected
  by an Evidence Window.  Values pool 16 complete formal runs.}
  \label{fig:evidence_lifecycle}
\end{figure*}


==> experiment/formal_exp_all_real.tex <==
% Requires: \usepackage{booktabs,tabularx,array,xcolor,colortbl}
% All deltas are absolute percentage-point changes relative to the No-skill
% result for the same action model and dataset, computed from integer counts.
\providecommand{\method}{\textsc{EviSkill}}
\providecommand{\bestresult}[1]{\textbf{#1}}
\providecommand{\secondresult}[1]{\underline{#1}}
\definecolor{eviskillblue}{RGB}{232,242,255}

\begin{table}[t]
\caption{Task-success accuracy (\%) across three interactive benchmarks. $\Delta_{\mathrm{NS}}$ denotes the percentage-point change relative to NoSkill for the same model and dataset. \textbf{Bold} and \underline{underlined} values indicate the best and second-highest distinct accuracies within each model--dataset setting}
\label{tab:main-results}
\centering
\fontsize{6.0}{6.8}\selectfont
\setlength{\tabcolsep}{1.0pt}
\renewcommand{\arraystretch}{1.02}
\begin{tabularx}{\columnwidth}{@{}
>{\hsize=1.35\hsize\raggedright\arraybackslash}X
>{\hsize=.95\hsize\raggedright\arraybackslash}X
*{6}{>{\hsize=.95\hsize\raggedleft\arraybackslash}X}@{}}
\toprule
\multirow[c]{2}{*}{Model} &
\multirow[c]{2}{*}{Method} &
\multicolumn{2}{c}{ALFWorld (134)} &
\multicolumn{2}{c}{AppWorld (168)} &
\multicolumn{2}{c}{ScienceWorld (211)} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
& & Acc.$\uparrow$ & $\Delta_{\mathrm{NS}}$ &
Acc.$\uparrow$ & $\Delta_{\mathrm{NS}}$ &
Acc.$\uparrow$ & $\Delta_{\mathrm{NS}}$ \\
\midrule
\multirow{7}{*}{\centering GPT-5.5}
 & No skill & 90.30 & 0.00 & 85.71 & 0.00 & 76.30 & 0.00 \\
 & LLM skill & 94.03 & +3.73 & \secondresult{94.05} & +8.33 & 76.78 & +0.47 \\
 & Trace2Skill & 94.03 & +6.72 & 86.31 & +0.60 & 65.40 & -10.90 \\
 & EvoSkill & 94.78 & +4.48 & 91.07 & +5.36 & 54.50 & -21.80 \\
 & SkillGrad & \secondresult{95.52} & +5.22 & 86.31 & +0.60 & 67.30 & -9.00 \\
 & SkillOpt & 94.78 & +4.48 & 92.86 & +10.71 & \secondresult{80.09} & +9.48 \\
\rowcolor{eviskillblue}
 & \method{} & \bestresult{96.27} & +5.97 & \bestresult{94.64} & -- & \bestresult{83.41} & +7.11 \\
\addlinespace[1.0pt]
\multirow{7}{*}{\centering GPT-5.4}
 & No skill & 75.37 & 0.00 & 88.10 & 0.00 & 52.13 & 0.00 \\
 & LLM skill & 89.55 & +14.18 & \bestresult{88.69} & +2.38 & \secondresult{66.35} & +14.22 \\
 & Trace2Skill & \secondresult{94.78} & +19.40 & 85.71 & -2.38 & 56.40 & +4.27 \\
 & EvoSkill & 90.30 & +14.93 & 79.17 & -8.93 & 63.03 & +10.90 \\
 & SkillGrad & 94.03 & +18.66 & 83.93 & -4.17 & 53.55 & +1.42 \\
 & SkillOpt & \secondresult{94.78} & +19.40 & \secondresult{89.29} & +1.19 & 63.03 & +10.90 \\
\rowcolor{eviskillblue}
 & \method{} & \bestresult{95.52} & +20.15 & \bestresult{90.48} & +2.38 & \bestresult{76.78} & +24.64 \\
\addlinespace[1.0pt]
\multirow{7}{*}{\centering GPT-5.4-mini}
 & No skill & 74.63 & 0.00 & 82.14 & 0.00 & 38.86 & 0.00 \\
 & LLM skill & 88.06 & +13.43 & 76.19 & -5.95 & 36.97 & -1.90 \\
 & Trace2Skill & 82.84 & +8.21 & 83.33 & +5.36 & 42.65 & +3.79 \\
 & EvoSkill & 86.57 & +11.94 & \bestresult{85.12} & +2.98 & 44.55 & +5.69 \\
 & SkillGrad & 88.06 & +13.43 & 83.33 & +1.19 & 44.08 & +5.21 \\
 & SkillOpt & \secondresult{89.55} & +14.93 & \secondresult{84.52} & +4.17 & \secondresult{58.29} & +19.43 \\
\rowcolor{eviskillblue}
 & \method{} & \bestresult{91.79} & +17.16 & 83.93 & +1.79 & \bestresult{67.78} & +28.91 \\
\addlinespace[1.0pt]
\multirow{7}{*}{\centering Qwen3.5-4B}
 & No skill & 43.28 & 0.00 & 18.45 & 0.00 & 4.27 & 0.00 \\
 & LLM skill & 75.37 & +32.09 & 28.57 & +10.12 & 3.79 & -0.47 \\
 & Trace2Skill & 82.84 & +39.55 & 32.14 & -- & 9.48 & +5.21 \\
 & EvoSkill & 73.88 & +30.60 & 27.98 & +9.52 & 2.84 & -1.42 \\
 & SkillGrad & \secondresult{84.33} & +41.79 & 30.36 & -- & 6.64 & +2.37 \\
 & SkillOpt & 83.58 & +41.04 & \secondresult{30.95} & +14.88 & \secondresult{14.69} & +10.43 \\
\rowcolor{eviskillblue}
 & \method{} & \bestresult{85.07} & +41.79 & \bestresult{32.14} & +13.69 & \bestresult{20.85} & +16.59 \\
\addlinespace[1.0pt]
\multirow{7}{*}{\centering Qwen3.5-9B}
 & No skill & 54.48 & 0.00 & 25.60 & 0.00 & 8.53 & 0.00 \\
 & LLM skill & 76.12 & +21.64 & 43.45 & +17.86 & 9.00 & +0.47 \\
 & Trace2Skill & 75.37 & +20.90 & 45.24 & -- & 19.91 & +11.37 \\
 & EvoSkill & 76.87 & +22.39 & 32.74 & -- & 17.06 & +8.53 \\
 & SkillGrad & \secondresult{87.31} & +32.84 & \secondresult{46.43} & -- & 14.22 & +5.69 \\
 & SkillOpt & 86.57 & +32.09 & \bestresult{47.62} & +24.40 & \secondresult{22.27} & +13.74 \\
\rowcolor{eviskillblue}
 & \method{} & \bestresult{91.04} & +36.57 & 43.45 & +17.86 & \bestresult{37.91} & +29.38 \\
\addlinespace[1.0pt]
\multirow{7}{*}{\centering \shortstack{Qwen3.6-35B-\\A3B}}
 & No skill & 70.90 & 0.00 & 54.17 & 0.00 & 17.06 & 0.00 \\
 & LLM skill & 79.85 & +8.96 & 58.33 & +4.17 & 17.54 & +0.47 \\
 & Trace2Skill & 85.07 & +14.18 & \bestresult{64.88} & +13.69 & 25.12 & +8.06 \\
 & EvoSkill & 79.85 & +8.96 & 55.36 & +1.19 & 23.22 & +6.16 \\
 & SkillGrad & 85.82 & +17.91 & 60.71 & -- & 19.91 & +2.84 \\
 & SkillOpt & \secondresult{86.57} & +17.91 & 62.50 & +8.33 & \bestresult{42.18} & +28.91 \\
\rowcolor{eviskillblue}
 & \method{} & \bestresult{88.06} & +17.16 & \secondresult{63.10} & +8.93 & \secondresult{40.76} & +23.70 \\
\bottomrule
\end{tabularx}
\vspace{1.5pt}
\end{table}


==> experiment/rejection_recovery.tex <==
% Rejection-aligned validation dynamics and post-rejection source-edit fate.
\subsection{Cross-Epoch Recovery after Global Rejection}
\label{sec:rejection_recovery_dynamics}

The preceding replay audit establishes that locally supported edits can survive
a candidate-level rejection.  We next ask whether a rejected run subsequently
recovers on validation and what happens to the source edits that pass
post-rejection replay.  Both analyses use the same frozen manifest of 16
complete runs and 64 epochs as the other mechanism audits.

\paragraph{Protocol and estimands.}
Let $\widetilde{S}_{r,e}$ be the full candidate revision submitted to global
validation by run $r$ at epoch $e$.  For every nonterminal rejection
$(r,e)$, we compute the rejection-aligned change
\begin{equation}
  \Delta^{\mathrm{next}}_{r,e}
  =100\!\left[
    \operatorname{Acc}_{\mathrm{val}}(\widetilde{S}_{r,e+1})
    -\operatorname{Acc}_{\mathrm{val}}(\widetilde{S}_{r,e})
  \right],
  \label{eq:rejection_aligned_recovery}
\end{equation}
in percentage points.  This is a validation-only diagnostic: the test split is
not evaluated at intermediate epochs.  We observe 29 global rejections, of
which 18 are eligible for Equation~\ref{eq:rejection_aligned_recovery}; the 11
epoch-4 rejections are structurally excluded because no next epoch exists.
Every eligible rejection is retained irrespective of whether its resulting
Provisional ledger is empty.  We show event-level changes, dataset medians, and
the event-weighted mean with a 95\% percentile interval from 50,000 bootstrap
resamples clustered by run.

For the second analysis, the cohort comprises 97 replay-accepted source-edit
events (92 direct accepts and 5 reflection-resolved accepts).  We follow each
source identifier through the final Provisional and validated records,
including descendants recorded in \texttt{merged\_from}.  Of these source
events, 96 are represented in the
Provisional ledger; two pairs later coalesce into shared records, yielding 94
distinct physical ledger records.  One reflected source edit passes replay but
fails patch application during reconciliation and is recorded separately as a
reconciliation failure.  A lineage is \emph{promoted} when it, or its tracked
descendant, is represented in a later globally committed revision.  Lineages
still live after epoch 4 are right-censored rather than treated as failures.

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{Figure/rejection_recovery.pdf}
  \caption{Cross-epoch dynamics after candidate-level rejection.
  (a) Paired validation accuracies for each nonterminal rejection event: the
  open gray endpoint is the rejected candidate at epoch $e$, the colored
  endpoint is the candidate submitted at epoch $e+1$, and the connecting line
  makes the direction of change explicit.  Endpoint labels report
  ``rejected $\to$ next'' accuracy; filled and hollow colored endpoints denote
  whether the next candidate is committed or rejected, respectively.  The
  header reports the event-weighted mean and its 95\% run-cluster bootstrap
  interval.  Final-epoch rejections are excluded because they have no
  next-epoch observation.  (b) Fate of replay-accepted
  source-edit events, with coalesced descendants followed
  through \texttt{merged\_from}.  The single reconciliation failure never
  becomes a live ledger record.  Active-at-horizon source events are
  administratively right-censored.  The panels have different units---18
  rejection events in (a) and 97 replay-accepted source-edit events in (b)---and
  constitute a descriptive mechanism audit rather than an isolated causal
  estimate.}
  \label{fig:rejection_recovery}
\end{figure*}

\paragraph{Next-submission recovery.}
Figure~\ref{fig:rejection_recovery}(a) connects the rejected and next candidate
directly, so the direction of each event is visible before taking any aggregate.
Validation accuracy increases
after 13 of the 18 eligible rejections, is unchanged after two, and decreases
after three.  The median change is $+2.80$ percentage points and the mean is
$+4.18$ points (95\% run-cluster bootstrap interval
$[+1.75,+7.11]$); eight of the next candidates pass the global gate.  The
dataset medians are $0.00$, $+10.53$, and $+4.17$ points on ALFWorld,
AppWorld, and ScienceWorld, respectively, indicating substantial descriptive
heterogeneity rather than uniform recovery.

\paragraph{Fate of replay-accepted source edits.}
Figure~\ref{fig:rejection_recovery}(b) tracks the 97-source-edit event cohort.
In total, 45 source events (46.39\%) are represented in a globally promoted revision
one epoch after admission and another 10 (10.31\%) are promoted after two
epochs.  Thus, 55 source events (56.70\%) are eventually represented in a promoted
bundle.  A further 41 (42.27\%) remain active at the four-epoch horizon, and
one (1.03\%) fails reconciliation.  The active group is an administrative
right-censoring category: it is neither a rejection nor evidence that those
edits would ultimately be promoted.

\paragraph{Interpretation and limitation.}
Together, the two panels show that a global rejection does not unconditionally
erase all cross-epoch information: replay-accepted source edits are often
carried forward, and the next submitted candidate frequently recovers
validation accuracy.  They do not identify the Provisional mechanism as the
sole cause of that change.  The next candidate combines the reconciled ledger
with newly collected Evidence Cards and newly generated edits, while the
analysis conditions on a low-performing rejected submission and is therefore
susceptible to selection and regression-to-the-mean effects.  Moreover, global
promotion validates an edit bundle, not an individual edit in isolation.
Causal support for Cross-Epoch Evidence Propagation therefore comes from the
controlled ablation in Section~\ref{sec:ablation}, not from this aligned audit
alone.


==> experiment/replay_model_breakdown.tex <==
% Per-model replay analysis. Percent signs are omitted inside the table.
\section{Per-model Replay Breakdown}
\label{app:replay_breakdown}

The following table reports replay outcomes for every available
dataset--backbone cell.  It is provided as an appendix audit; the main text
uses the aggregate replay panels in Figure~\ref{fig:replay_edit_outcomes}.

\begin{table}[!ht]
\caption{Replay outcomes by dataset and Action-Agent backbone.  $A$, $F$, and
$R^{*}$ denote initial accept, reflect, and reject-or-defer shares; Ret. and
Adm. denote final retention and Provisional admission.  Entries are percentages
and $n$ is the number of replayed edits.  N/A indicates that post-rejection
replay was structurally unavailable at the final epoch or because no rejection
occurred.}
\label{tab:replay_model_breakdown}
\centering
\scriptsize
\setlength{\tabcolsep}{3.4pt}
\renewcommand{\arraystretch}{1.04}
\begin{tabular}{@{}llrrrrr@{\qquad}rrrrr@{}}
\toprule
Dataset & Model &
\multicolumn{5}{c}{Evidence-window replay} &
\multicolumn{5}{c}{Post-rejection replay} \\
\cmidrule(lr){3-7}\cmidrule(lr){8-12}
 & & $n$ & $A$ (\%) & $F$ (\%) & $R^{*}$ (\%) & Ret. (\%) &
 $n$ & $A$ (\%) & $F$ (\%) & $R^{*}$ (\%) & Adm. (\%) \\
\midrule
ALFWorld & GPT-5.4          & 28 & 85.71 & 0.00 & 14.29 & 85.71 & 7 & 71.43 & 0.00 & 28.57 & 71.43 \\
ALFWorld & GPT-5.4-mini     & 27 & 59.26 & 0.00 & 40.74 & 59.26 & 6 & 66.67 & 0.00 & 33.33 & 66.67 \\
ALFWorld & GPT-5.5          & 18 & 77.78 & 0.00 & 22.22 & 77.78 & 2 & 100.00 & 0.00 & 0.00 & 100.00 \\
ALFWorld & Qwen3.5-9B       & 22 & 81.82 & 4.55 & 13.64 & 86.36 & 8 & 87.50 & 0.00 & 12.50 & 87.50 \\
ALFWorld & Qwen3.6-35B-A3B  & 21 & 95.24 & 0.00 & 4.76 & 95.24 & 9 & 100.00 & 0.00 & 0.00 & 100.00 \\
\addlinespace[1.5pt]
AppWorld & GPT-5.4          & 44 & 86.36 & 4.55 & 9.09 & 90.91 & 8 & 100.00 & 0.00 & 0.00 & 100.00 \\
AppWorld & GPT-5.4-mini     & 46 & 76.09 & 6.52 & 17.39 & 80.43 & 2 & 50.00 & 0.00 & 50.00 & 50.00 \\
AppWorld & Qwen3.5-4B       & 68 & 57.35 & 4.41 & 38.24 & 61.76 & 14 & 57.14 & 21.43 & 21.43 & 71.43 \\
AppWorld & Qwen3.5-9B       & 81 & 41.98 & 7.41 & 50.62 & 46.91 & 13 & 53.85 & 0.00 & 46.15 & 53.85 \\
AppWorld & Qwen3.6-35B-A3B  & 67 & 47.76 & 2.99 & 49.25 & 50.75 & 12 & 58.33 & 8.33 & 33.33 & 66.67 \\
\addlinespace[1.5pt]
ScienceWorld & GPT-5.4         & 115 & 64.35 & 10.43 & 25.22 & 73.91 & 11 & 81.82 & 9.09 & 9.09 & 81.82 \\
ScienceWorld & GPT-5.4-mini    & 159 & 49.06 & 9.43 & 41.51 & 57.86 & 21 & 52.38 & 4.76 & 42.86 & 57.14 \\
ScienceWorld & GPT-5.5         & 103 & 60.19 & 4.85 & 34.95 & 65.05 & \multicolumn{5}{c}{\textit{N/A: final epoch}} \\
ScienceWorld & Qwen3.5-4B      & 125 & 90.40 & 5.60 & 4.00 & 94.40 & 15 & 93.33 & 0.00 & 6.67 & 93.33 \\
ScienceWorld & Qwen3.5-9B      & 116 & 38.79 & 6.90 & 54.31 & 44.83 & \multicolumn{5}{c}{\textit{N/A: final epoch}} \\
ScienceWorld & Qwen3.6-35B-A3B & 132 & 44.70 & 5.30 & 50.00 & 50.00 & \multicolumn{5}{c}{\textit{N/A: no reject}} \\
\bottomrule
\end{tabular}
\end{table}


==> sections/1.Introduction_old.tex <==
\section{Introduction}

Large language model (LLM) agents increasingly rely on external skills to solve interactive tasks such as tool use, web navigation, and long-horizon decision making. These skills encode task procedures, tool-use rules, and recovery strategies in natural language, allowing agents to reuse procedural knowledge without modifying model parameters. However, skills created before deployment inevitably provide only partial coverage of the situations an agent may encounter, as subsequent interactions continually expose new states, operational constraints, and failure cases. This has motivated continual skill evolution, where interaction trajectories are repeatedly converted into reusable experience and written back into the external skill \citep{skilladaptor2026,trace2skill2026,skillgrad2026,coevolveskill2026,codeskill2026,skillr12026,skillx2026}. Modern skill-evolution pipelines therefore involve more than generating a single update: they identify useful experience, produce one or more edits, combine these edits into a revised skill, and increasingly evaluate the complete revision before deciding whether to commit it \citep{evoskill2026,skillopt2026}. Such global validation is important because locally motivated edits may interact with one another or degrade behavior on other tasks. However, \textbf{when a complete skill revision fails global validation, should all of the progress contained within that revision be discarded?}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{Figure/motivation.pdf}
  \caption{xxx}
  \label{fig:framework}
\end{figure}


Figure~\ref{fig:motivation} illustrates the failure mode behind this question. A candidate revision may contain several edits supported by different interaction experiences, yet aggregate validation produces only a decision on the complete revised skill. A rejection therefore reveals that the current combination should not be promoted, but does not by itself establish that every constituent edit is invalid. In pipelines that apply whole-revision rollback, this aggregate decision raises two concerns. \textbf{First, useful edits can be obscured by revision failure.} A revision may fail because only a subset of its edits is harmful, or because otherwise useful edits become incompatible when combined, causing locally supported edits to be discarded together with those responsible for the regression. \textbf{Second, whole-revision rollback can interrupt continual optimization.} Once these edits are removed from the executable skill, subsequent interactions can no longer further verify, refine, or correct them, and the system may encounter the same problems again and reconstruct similar updates from newly collected trajectories. Revision failure should therefore not be treated solely as a signal to reset the optimization process. Instead, it raises a more consequential question: \textbf{which parts of a failed revision remain sufficiently supported to contribute to subsequent evolution?}

Answering this question requires more than preserving edits that appeared locally successful. The behavioral evidence that motivated an edit must remain associated with it so that the edit can be revisited after merging and global rejection, while retained edits must remain distinguishable from globally validated progress because their effects may change as the surrounding skill evolves. Existing approaches address important pieces of this process, including fine-grained trajectory diagnosis \citep{skilladaptor2026}, cross-trajectory experience consolidation \citep{trace2skill2026}, matched execution-based assessment \citep{coevolveskill2026}, and validation-based revision selection \citep{evoskill2026,skillopt2026}, but they do not provide a continuous mechanism for carrying localized behavioral evidence together with supported edits across a rejected revision and using subsequent behavior to refine them. 

To address this challenge, we introduce \method{}, an evidence-grounded framework for continual skill evolution. \method{} constructs \emph{Replayable Evidence Cards} that bind localized trajectory segments to proposed skill changes, consolidates related evidence into skill edits, and evaluates these edits through trigger-range replay before global validation. When the resulting revision is rejected, \method{} keeps the previously Validated Skill unchanged while reexamining the constituent edits through their linked evidence and carrying supported or evidence-grounded corrected edits forward as \emph{Provisional Edits}. These edits remain executable in the next Candidate Skill, where subsequent trajectories provide additional evidence for their support or correction through \emph{Cross-Epoch Evidence Propagation}. In this way, revision failure no longer necessarily resets the evolution process, and previously supported progress can continue to participate in later optimization without being prematurely promoted as globally validated knowledge. After a fixed evolution budget, the latest globally validated skill is returned as the final evolved skill and is frozen for execution on unseen tasks.

Our contributions are summarized as follows:
\begin{itemize}
    \item \textbf{Rethinking revision failure.} We identify a limitation of whole-revision rollback in continual skill evolution: rejection of a complete revision does not imply that all of its constituent edits are invalid, and discarding them together can erase locally supported progress and interrupt subsequent optimization.

    \item \textbf{Evidence-grounded continual evolution.} We introduce \method{}, which maintains persistent links between localized behavioral evidence and skill edits through Replayable Evidence Cards, evaluates edits through trigger-range replay, and carries supported or corrected edits across revision failures as Provisional Edits for continued evaluation and refinement.

    \item \textbf{Evaluation and mechanism analysis.} We evaluate \method{} on AppWorld, ScienceWorld, and ALFWorld across multiple LLM agent backbones. Beyond overall task performance and controlled ablations, we analyze how edits and their supporting evidence survive global rejection, propagate across evolution epochs, and undergo subsequent reuse and correction.
\end{itemize}

==> sections/3.method_old.tex <==
\section{Method}
\label{sec:method}

As illustrated in Figure~\ref{fig:framework}, \method{} uses execution evidence to guide the synthesis, verification, and cross-epoch refinement of skill edits through three phases. \textbf{Evidence-Grounded Edit Synthesis} extracts Replayable Evidence Cards from execution trajectories and synthesizes localized edits grounded in their supporting trajectory segments. \textbf{Replay-Guided Edit Verification} re-executes the corresponding behaviors from the same starting contexts and uses replay outcomes to verify and refine the proposed edits. \textbf{Cross-Epoch Evidence Propagation} uses global validation to update the Validated Skill $S_e^V$, retain replay-supported Provisional Edits in the Working Skill $S_e^W$, and propagate relevant evidence for subsequent evolution.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{Figure/framework.pdf}
    \caption{Overview of \method{}.}
    \label{fig:framework}
\end{figure*}

\subsection{Evidence-Grounded Edit Synthesis}
\label{sec:edit_construction}

Distilling trajectories into procedural guidance can obscure the contexts that justify a correction. We construct each edit together with its source evidence, preserving a path to the behavior it targets.

\noindent\textbf{Definition 1 (Working Skill).} \textit{At epoch $e$, the Working Skill $S_e^W$ combines the latest Validated Skill $S_e^V$ with the Provisional Edit Ledger $P_e$, an ordered collection of replay-supported edits not yet incorporated into $S_e^V$:}
\begin{equation} S_e^W=S_e^V\oplus P_e. \label{eq:working_skill} \end{equation}
\textit{Here, $\oplus$ applies the edits in order, and each entry in $P_e$ retains its supporting evidence references. The validation-gated update of $P_e$ is described in Section~\ref{sec:evidence_propagation}. Initially, $S_1^V=S_0$ and $P_1=\varnothing$, so $S_1^W=S_0$.}

The Action Agent $\pi$ collects one trajectory $\tau_x^e\sim\pi(\cdot\mid x,S_e^W)$ for each training task $x\in\mathcal{D}_{\mathrm{tr}}$, and $\mathcal{R}_e$ denotes the resulting trajectory set.

\textbf{Evidence extraction and grounding.} An LLM evidence extractor $f_{\phi}^{\mathrm{ext}}$ analyzes the current Working Skill $S_e^W$ and trajectories $\mathcal{R}_e$ to identify behaviors that motivate changes to the skill's procedures, preconditions, or recovery guidance, and associates each proposed correction with the trajectory intervals that support it.

\noindent\textbf{Definition 2 (Replayable Evidence Card).} \textit{A Replayable Evidence Card associates a proposed skill correction with its supporting execution evidence:}
\begin{equation} C_i=\langle z_i,\mathcal{G}_i,\widetilde{u}_i\rangle, \label{eq:evidence_card} \end{equation}
\textit{where $z_i$ is a persistent identifier, $\mathcal{G}_i$ is a set of supporting trigger ranges, and $\widetilde{u}_i$ is the proposed correction. Each trigger range $g=(x,e_g,s,t)$ identifies the interval $[s,t]$ in the source trajectory $\tau_x^{e_g}$ of task $x$ at source epoch $e_g$. A Card may contain multiple ranges from the same or different tasks when they support the same correction.}

Applying $f_{\phi}^{\mathrm{ext}}$ to $S_e^W$ and $\mathcal{R}_e$ produces the Trajectory Evidence Cards $\mathcal{C}_e^{\mathrm{traj}}=f_{\phi}^{\mathrm{ext}}(S_e^W,\mathcal{R}_e)$, which capture behaviors and potential improvements identified in the current trajectories.

For cross-epoch evidence, let $\mathcal{Q}_e$ denote the Tracked Edits, with $\mathcal{Q}_1=\varnothing$. For $e>1$, $\mathcal{Q}_e$ contains the live Provisional Edits in $P_e$ and the edits newly incorporated into $S_e^V$ during the preceding epoch transition. Let $\mathcal{X}_e$ denote the training tasks referenced by their supporting Cards, and let $\mathcal{R}_e^{\mathrm{cmp}}$ collect the complete trajectory pairs $(\tau_x^{e-1},\tau_x^e)$ for $x\in\mathcal{X}_e$. The evidence extractor then produces the Contrastive Evidence Cards $\mathcal{C}_e^{\mathrm{con}}=f_{\phi}^{\mathrm{ext}}(S_e^W,\mathcal{Q}_e,\mathcal{R}_e^{\mathrm{cmp}})$ for $e>1$. These Cards identify persistent deficiencies or newly exposed problems and retain links to their supporting trajectory ranges and, when applicable, the existing edits they target.

Writing $\mathcal{C}_e^{\mathrm{carry}}$ for the Cards preserved after the preceding validation and lifecycle updates, the Evidence Pool available for edit construction is: 
\begin{equation} \mathcal{C}_e=\mathcal{C}_e^{\mathrm{carry}}\cup\mathcal{C}_e^{\mathrm{traj}}\cup\mathcal{C}_e^{\mathrm{con}}. \label{eq:evidence_propagation} \end{equation}
At the first epoch, $\mathcal{C}_1^{\mathrm{carry}}=\mathcal{C}_1^{\mathrm{con}}=\varnothing$, so Eq.~\ref{eq:evidence_propagation} reduces to $\mathcal{C}_1=\mathcal{C}_1^{\mathrm{traj}}$. Section~\ref{sec:evidence_propagation} describes how lifecycle updates determine $\mathcal{C}_{e+1}^{\mathrm{carry}}$.

\textbf{Evidence grouping and edit synthesis.} We organize active Cards with compatible source contexts and correction intents into Evidence Windows, where $\mathcal{B}_k=\{C_i\}_{i\in\mathcal{I}_k}\subseteq\mathcal{C}_e$ denotes the $k$-th Window for $k=1,\ldots,K_e$. Given $S_e^W$ and $\mathcal{B}_k$, an LLM editor $f_{\psi}^{\mathrm{edit}}$ refines or consolidates the Card-level proposals into localized candidate edits:
\begin{equation} \mathcal{U}_e=\bigcup_{k=1}^{K_e}f_{\psi}^{\mathrm{edit}}\!\left(S_e^W,\mathcal{B}_k\right). \label{eq:candidate_edits} \end{equation}
Each edit $u\in\mathcal{U}_e$ retains the identifiers $I_u$ of its supporting Cards, with the associated replay ranges given by $\mathcal{G}(u)=\bigcup_{i:z_i\in I_u}\mathcal{G}_i$. These evidence links provide the source contexts used to replay and verify each candidate edit.

\subsection{Replay-Guided Edit Verification}
\label{sec:edit_verification}

An edit may be grounded in its source evidence yet fail to correct the corresponding behavior. We verify candidate edits through re-execution and use replay outcomes to assess and refine them.

\textbf{Behavioral verification.} For each candidate edit $u$, we retrieve its supporting Cards $\mathcal{C}(u)=\{C_i\in\mathcal{C}_e\mid z_i\in I_u\}$ and replay the trigger ranges in $\mathcal{G}(u)$. For each range $g=(x,e_g,s,t)$, we reproduce the prefix of $\tau_x^{e_g}$ preceding step $s$ to reconstruct the source execution state and interaction history. From this context, the Action Agent $\pi$ re-executes the segment $[s,t]$ under $S_e^W\oplus u$ to determine whether the intended correction is achieved without introducing new failures.

An LLM evaluator $f_{\theta}^{\mathrm{eval}}$ compares each replayed segment with its source counterpart. Let $\mathcal{T}_u$ denote the resulting source--replay segment pairs for the trigger ranges in $\mathcal{G}(u)$, where $\tau_g^{\mathrm{src}}$ is the source segment specified by $g$ and $\tau_g^{\mathrm{rep}}$ is generated under $S_e^W\oplus u$ from the same starting context. The evaluator assesses these pairs with the edit and its supporting Cards:
\begin{equation} (r_u,h_u)=f_{\theta}^{\mathrm{eval}}\!\left(S_e^W,u,\mathcal{C}(u),\mathcal{T}_u\right). \label{eq:llm_replay_assessment} \end{equation}
Here, $r_u\in\{\mathrm{accept},\mathrm{reflect},\mathrm{reject}\}$ is the replay decision and $h_u$ is the corresponding feedback. The evaluator $f_{\theta}^{\mathrm{eval}}$ assigns \emph{accept} when replay supports the correction, \emph{reflect} when a localized deficiency can guide revision, and \emph{reject} otherwise. For $r_u=\mathrm{reflect}$, the LLM editor produces the corrected edit $u'=f_{\psi}^{\mathrm{edit}}(S_e^W,u,\mathcal{C}(u),\mathcal{T}_u,h_u)$. The corrected edit retains its evidence links and undergoes another replay and evaluation.

\textbf{Verified edit consolidation.} The replay-verified edits are given by:
\begin{equation} \mathcal{U}_e^{+}=\{u\in\mathcal{U}_e\mid r_u=\mathrm{accept}\}\cup\{u'\mid u\in\mathcal{U}_e,\ r_u=\mathrm{reflect},\ r_{u'}=\mathrm{accept}\}. \label{eq:verified_edits} \end{equation}
Edits without acceptance are excluded from the current candidate, while their supporting Cards remain available for subsequent proposals. The LLM editor consolidates the compatible edits into the ordered set $\overline{\mathcal{U}}_e=f_{\psi}^{\mathrm{edit}}(S_e^W,\mathcal{U}_e^{+})$ while preserving their supporting Card associations. Applying these edits to the Working Skill produces the candidate revision $\widetilde{S}_e=S_e^W\oplus\overline{\mathcal{U}}_e$.

\subsection{Cross-Epoch Evidence Propagation}
\label{sec:evidence_propagation}
To preserve information that can support further evolution, we carry unresolved Cards across epochs for reuse in subsequent edit construction. When a revision is rejected, edits supported by post-rejection replay are also retained provisionally in the next Working Skill for continued training interactions and refinement, while the Validated Skill remains unchanged, i.e., $S_{e+1}^V=S_e^V$.

\textbf{Validation-gated carryover.} Let $\widehat{J}_{\mathcal{D}_{\mathrm{val}}}(S)$ denote the empirical performance of skill $S$ on the validation set $\mathcal{D}_{\mathrm{val}}$. At epoch $e$, global validation updates the Validated Skill as follows:
\begin{equation} S_{e+1}^{V}=\begin{cases}\widetilde{S}_e, & \widehat{J}_{\mathcal{D}_{\mathrm{val}}}(\widetilde{S}_e)>\widehat{J}_{\mathcal{D}_{\mathrm{val}}}(S_e^V),\\ S_e^V, & \text{otherwise}.\end{cases} \label{eq:validated_skill_update} \end{equation}
If $\widetilde{S}_e$ is accepted, the Provisional Edits in $P_e$ and the consolidated edits in $\overline{\mathcal{U}}_e$ are incorporated into $S_{e+1}^V$, the Provisional Edit Ledger is cleared as $P_{e+1}=\varnothing$, and the next Tracked Edits are set to $\mathcal{Q}_{e+1}=P_e\cup\overline{\mathcal{U}}_e$. Their supporting Card references are retained for cross-epoch comparison. If $\widetilde{S}_e$ is rejected, $S_{e+1}^V=S_e^V$, and each consolidated edit $v\in\overline{\mathcal{U}}_e$ undergoes post-rejection replay using its preserved Card associations. The LLM evaluator $f_{\theta}^{\mathrm{eval}}$ returns a post-rejection decision $r_v^{\mathrm{post}}$, while edits assigned \emph{reflect} are revised by the LLM editor $f_{\psi}^{\mathrm{edit}}$ and replayed once more. The replay-retained forms are: 
\begin{equation} \mathcal{U}_e^{\mathrm{post},+}=\{v\in\overline{\mathcal{U}}_e\mid r_v^{\mathrm{post}}=\mathrm{accept}\}\cup\{v'\mid v\in\overline{\mathcal{U}}_e,\ r_v^{\mathrm{post}}=\mathrm{reflect},\ r_{v'}^{\mathrm{post}}=\mathrm{accept}\}. \label{eq:post_rejection_retained_edits} \end{equation}
The edits in $\mathcal{U}_e^{\mathrm{post},+}$ update $P_e$ by replacing the entries they target and appending the remaining edits in order, yielding $P_{e+1}$ and the next Tracked Edits $\mathcal{Q}_{e+1}=P_{e+1}$. The next epoch uses $S_{e+1}^W=S_{e+1}^V\oplus P_{e+1}$, keeping provisional guidance available for training while maintaining the separate Validated Skill $S_{e+1}^V$.

\textbf{Evidence reuse and correction.} We update Card availability in the Evidence Pool according to validation and replay outcomes. Active Cards remain available for edit construction. Cards supporting live Provisional Edits are marked as protected: their task and trajectory references are preserved for cross-epoch comparison and corrective evidence generation, while they are excluded from new Evidence Windows. If $\widetilde{S}_e$ is accepted, Cards supporting the edits incorporated into $S_{e+1}^{V}$ are archived and excluded from new Evidence Windows, while their source references remain available for cross-epoch comparison. Repeated replay rejection can transition active Cards to stale.

These lifecycle updates determine the carried evidence $\mathcal{C}_{e+1}^{\mathrm{carry}}$. At the next epoch, Section~\ref{sec:edit_construction} uses $S_{e+1}^W$ to collect new training trajectories and extract trajectory and Contrastive Evidence Cards. Together with the carried evidence, these Cards form $\mathcal{C}_{e+1}$ through Eq.~\ref{eq:evidence_propagation} and support further edit construction and correction.

After $E$ evolution epochs, the latest Validated Skill $S_{E+1}^V$ is frozen for inference:
\begin{equation} S^\star=S_{E+1}^V,\qquad \tau_x\sim\pi(\cdot\mid x,S^\star),\quad x\in\mathcal{D}_{\mathrm{test}}. \label{eq:final_skill_inference} \end{equation}
The execution agent uses $S^\star$ on unseen test tasks without further skill evolution. Unpromoted Provisional Edits are excluded, and neither the skill nor the Evidence Pool is updated from test outcomes.

==> sections/4.experiment_old.tex <==
\section{Experiments}
\label{sec:experiments}

Our experiments address three questions. \textbf{Q1 (Overall Performance):} How does \method{} compare with existing skill-evolution methods across different benchmarks and LLM backbones? \textbf{Q2 (Component Contribution):} How do trigger-range replay and cross-epoch evidence propagation contribute to task performance? \textbf{Q3 (Mechanism Analysis):} How does replay filter and refine edits, and how are evidence and supported edits reused across evolution epochs?

\subsection{Experimental Setting}
\label{sec:experimental_setting}

\paragraph{Datasets.} We evaluate \method{} on three interactive benchmarks: AppWorld~\citep{appworld} for task execution through application APIs, ScienceWorld~\citep{scienceworld} for scientific experimentation, and ALFWorld~\citep{alfworld} for household task execution in text-based environments. 

\paragraph{Baselines and Models.} We compare \method{} with two reference settings and four skill-evolution methods. \emph{NoSkill} executes tasks without external skills, while \emph{LLM Skill} uses an initial LLM-generated skill without further evolution. SkillOpt~\citep{skillopt2026} optimizes skill documents through bounded edits selected by held-out validation. Trace2Skill~\citep{trace2skill2026} extracts trajectory-local lessons and hierarchically consolidates them into reusable skills. SkillGrad~\citep{skillgrad2026} uses trajectory diagnoses as textual gradients and incorporates momentum to guide skill updates. EvoSkill~\citep{evoskill2026} discovers and refines skills through iterative failure analysis and validation-based selection. For task execution, we evaluate six LLM backbones from two model families: GPT-5.5, GPT-5.4, and GPT-5.4-mini~\citep{gpt_models}, together with Qwen3.6-35B-A3B, Qwen3.5-9B, and Qwen3.5-4B~\citep{qwen_models}.

\paragraph{Evaluation Metrics.} We report task-success accuracy (Acc., \%), defined as the percentage of test tasks that satisfy each benchmark's full success criterion. This metric measures whether the evolved skills support complete task execution on unseen tasks.

\paragraph{Implementation Details.}
\method{} uses four skill-evolution epochs, while baselines follow their released update schedules. Detailed experimental configurations are provided in Appendix~\ref{app:experimental_details}.

\subsection{Main Results}
\label{sec:overall_results}

Table~\ref{tab:main-results} compares task-success accuracy across three interactive benchmarks and six LLM backbones. \method{} achieves the best or tied-best result in 14 of the 18 model--dataset settings and ranks among the top two methods in 16. Relative to NoSkill, it improves accuracy in all 18 settings, with an average gain of 17.93 percentage points when each setting receives equal weight. The largest improvements occur on ALFWorld with Qwen3.5-4B and Qwen3.5-9B, reaching 41.79 and 36.57 points, respectively. Improvements also extend beyond the NoSkill comparison. On ScienceWorld, \method{} exceeds the strongest reported baseline by 15.64 points with Qwen3.5-9B and 10.43 points with GPT-5.4.

\input{experiment/formal_exp}

\subsection{Ablation Study}
\label{sec:ablation}

To answer Q2, we evaluate two controlled variants of \method{}:
\emph{w/o Replay}, which removes Trigger-Range Replay, and
\emph{w/o Cross-Epoch}, which disables Cross-Epoch Evidence Propagation,
preventing replay-supported edits and their evidence from being carried
forward after a rejected revision.
Figure~\ref{fig:ablation} reports hard-success accuracy averaged over
three backbones within each model family.

Both components contribute consistently at the family level.
For GPT models, removing replay reduces average accuracy by
2.49, 4.56, and 2.85 percentage points on ALFWorld, AppWorld, and
ScienceWorld, respectively, while removing Cross-Epoch Evidence
Propagation reduces it by 1.49, 4.16, and 1.11 points.
The same trend holds for Qwen models: the full framework outperforms
both ablations on all three benchmarks, with replay contributing
2.24, 3.17, and 0.47 points and Cross-Epoch Evidence Propagation
contributing 3.48, 1.78, and 1.58 points.
These results show that localized behavioral verification and
cross-epoch evidence reuse provide complementary benefits across
model families and environments.

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figure/gpt_family_ablation.pdf}
        \caption{GPT models.}
        \label{fig:ablation-gpt}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figure/qwen_family_ablation.pdf}
        \caption{Qwen models.}
        \label{fig:ablation-qwen}
    \end{subfigure}
    \caption{
    Component ablations averaged within model families.
    Each bar reports hard-success accuracy (\%) averaged over three GPT
    backbones or three Qwen backbones on the corresponding benchmark.
    \emph{w/o Replay} removes Trigger-Range Replay, while
    \emph{w/o Cross-Epoch} removes Cross-Epoch Evidence Propagation.
    }
    \label{fig:ablation}
\end{figure}

\subsection{Mechanism Analysis}
\label{sec:mechanism_analysis}

To answer Q3, we analyze 18 complete runs covering 72 skill-evolution epochs. We examine how replay filters and refines candidate edits, and how cross-epoch evidence propagation enables evidence reuse and the continued correction of retained edits.

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{Figure/replay_edit_outcomes.pdf}
  \caption{Replay decisions and reflection outcomes for evidence-window replay (top) and replay after global validation rejection (bottom). Left panels show initial decisions over all replayed edits. Right panels show the counts and percentages of recovered and non-retained edits among reflected edits only. Percentages are computed from pooled edit counts across runs and epochs within each benchmark.}
  \label{fig:replay_edit_outcomes}
\end{figure*}

\subsubsection{Replay-Guided Edit Verification}
\label{sec:evidence_grounded_mechanism_analysis}

\paragraph{Replay-based edit filtering.} Figure~\ref{fig:replay_edit_outcomes} shows that replay accepts most edits directly while filtering a substantial fraction of proposals. During evidence-window replay, rejected edits account for 36.6\% of the proposals on AppWorld and 35.3\% on ScienceWorld. Reflection provides an opportunity to revise initially unsupported edits, recovering 13 of 16 reflected edits on AppWorld and 49 of 54 on ScienceWorld. Following global validation rejection, 3 of 4 reflected edits on AppWorld and 1 of 2 on ScienceWorld are accepted after correction and retained. These outcomes illustrate how replay combines proposal filtering with feedback-guided edit correction.


\subsubsection{Cross-Epoch Evidence Propagation}
\label{sec:cross_epoch_mechanism_analysis}

\paragraph{Edit retention and promotion.} Edits from rejected revisions can still contribute to subsequent globally accepted skills. Figure~\ref{fig:cross_epoch_retention}(a) reports 97 post-rejection replay acceptances and 96 retained edits. Among the replay-accepted source edits, Figure~\ref{fig:cross_epoch_retention}(b) shows that 46.4\% are incorporated into the Validated Skill one epoch later and 10.3\% two epochs later. Their subsequent promotion demonstrates that preserving locally supported edits can carry progress from rejected revisions into later accepted skills. Another 42.3\% remain provisional at the end of the fourth epoch, leaving their eventual outcomes unobserved within the evolution budget.

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{Figure/cross_epoch_retention_lifecycle.pdf}
  \caption{Retention and promotion of edits from rejected revisions. (a) Aggregate edit-event counts at candidate generation, replay allocation, replay acceptance, and retention. Ledger includes source edits that remain provisional or are subsequently promoted. (b) Outcomes of replay-accepted source edits, with percentages computed within each row. +1/+2 promotion denotes incorporation into the Validated Skill after one or two epochs. Active at E4 indicates that an edit remains provisional when evolution ends. Failure denotes unsuccessful ledger reconciliation.}
  \label{fig:cross_epoch_retention}
\end{figure*}


\paragraph{Evidence lifecycle and cross-epoch reuse.}
We further examine how the evidence pool evolves across epochs and how long individual Cards continue to contribute to edit construction. Figure~\ref{fig:evidence_lifecycle}(a) shows the composition of each epoch's input pool in terms of archived, stale, and active Cards. Archived evidence accounts for the largest share in most epochs, while the active share varies substantially and peaks at 50.0\% in Epoch~3; stale evidence remains consistently limited (\(\leq 6.6\%\)). Figure~\ref{fig:evidence_lifecycle}(b) summarizes the persistence depth of unique Evidence Cards across benchmarks. Overall, 54.3\% of Cards are selected in one epoch, whereas 23.0\% are reused across at least two epochs, indicating that a non-negligible fraction of evidence continues to support edit construction beyond its first use. The benchmark-level distributions further reveal different reuse patterns: ALFWorld contains a large fraction of pre-resolved evidence, while AppWorld and ScienceWorld exhibit substantially more evidence persisting across one or two evolution epochs.

\begin{figure*}[t]
  \centering

  \begin{subfigure}[t]{0.46\textwidth}
    \centering
    \includegraphics[width=\linewidth]{Figure/evidence_lifecycle_a.pdf}
    \caption{}
    \label{fig:evidence_lifecycle_pool}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.52\textwidth}
    \centering
    \includegraphics[width=\linewidth]{Figure/evidence_lifecycle_b.pdf}
    \caption{}
    \label{fig:evidence_lifecycle_depth}
  \end{subfigure}

  \caption{
  Evidence lifecycle and cross-epoch reuse over four evolution epochs.
  (a) Evolution of the epoch input pool, showing the percentages of archived,
  stale, and active Cards, pooled across 18 runs.
  (b) Persistence-depth distribution of unique Evidence Cards for each benchmark
  and their count-weighted aggregate (\emph{All}).
  \emph{Pre-resolved} denotes Cards resolved before any cross-epoch
  Evidence-Window assignment, while \(k\) epochs denotes Cards selected for
  Evidence Windows in \(k\) distinct epochs.
  Percentages in (b) are computed within each row.
  }
  \label{fig:evidence_lifecycle}
\end{figure*}

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\textwidth]{Figure/evidence_lifecycle.pdf}
%   \caption{Evidence lifecycle and reuse over four evolution epochs. (a) Archived, stale, and active Cards as percentages of each epoch's input pool, pooled across 18 runs. (b) Distribution of the number of distinct epochs in which each Card is selected for an Evidence Window, computed over unique Cards within each benchmark. Not selected denotes Cards never selected during the four epochs.}
%   \label{fig:evidence_lifecycle}
% \end{figure*}

Per-model replay outcomes are tabulated in Appendix~\ref{app:replay_breakdown};
N/A denotes that post-rejection replay was not executable for that cell.
The contrastive correction audit is reported in Appendix~\ref{app:contrastive_rewrite}.


==> sections/experiment_old.tex <==
\section{Experiments}
\label{sec:experiments}

Our experiments address three questions. \textbf{Q1 (Overall Performance):} How does \method{} compare with existing skill-evolution methods across different benchmarks and LLM backbones? \textbf{Q2 (Component Contribution):} How do trigger-range replay and cross-epoch evidence propagation contribute to task performance? \textbf{Q3 (Mechanism Analysis):} How does replay filter and refine edits, and how are evidence and supported edits reused across evolution epochs?

\subsection{Experimental Setting}
\label{sec:experimental_setting}

\paragraph{Datasets.}
We evaluate \method{} on three interactive benchmarks: AppWorld, ScienceWorld,
and ALFWorld.  AppWorld contains 90 training, 57 development, and 168 test
tasks; ScienceWorld contains 96 training, 48 development, and 211 test tasks;
and ALFWorld contains 96 training, 48 development, and 134 test tasks.  The
training split supplies interaction evidence, the development split is used
only for global validation and skill selection, and the test split remains
untouched until final evaluation.

\paragraph{Datasets.} We evaluate \method{} on three interactive benchmarks: AppWorld~\citep{appworld2024} for task execution through application APIs, ScienceWorld~\citep{scienceworld2022} for scientific experimentation, and ALFWorld~\citep{alfworld2021} for household task execution in text-based environments. 

\paragraph{Baselines.}
We compare \method{} with NoSkill, the unevolved LLM Skill, SkillOpt,
Trace2Skill, SkillGrad, and EvoSkill.  We freeze one result per
method--model--dataset cell and do not select the best score across repeated
runs.  Numeric inclusion follows the current frozen Acc snapshot; ``--'' marks
a cell for which that snapshot retains no reportable value.  The August 26--27
AppWorld reruns replace the historical GPT NoSkill and SkillOpt results and add
complete GPT-5.5/GPT-5.4 Trace2Skill and SkillGrad results.  The frozen
GPT-5.5 LLM-skill summary reports 158/168 while one task ended with an
unrecovered HTTP 502; we retain the reported full-split summary and disclose
this caveat.  For GPT-5.4-mini, a newer initial-skill retry had 107 HTTP 429
failures, so the snapshot instead retains the earlier error-free 128/168
evaluation.

\paragraph{Evaluation Metrics.}
We use test hard-success accuracy as the primary metric.  Where an environment
provides graded rewards, average task score measures partial progress;
ALFWorld's score is binary under our protocol and therefore equals accuracy.

\paragraph{Implementation Details.}
\method{} uses four skill-evolution epochs and seed 42; baselines follow their
released update schedules.  All AppWorld GPT evaluations use a 4096-token
action cap and medium reasoning.  For Qwen, \method{}, LLM Skill, SkillOpt, and
the newly aligned Qwen3.6-35B-A3B Trace2Skill/EvoSkill reruns use a 2048-token
cap, whereas NoSkill, the latest Qwen3.5-4B/9B Trace2Skill reruns, and several
retained legacy baseline rows use 4096.  The accumulated campaign also contains
two initial-skill cohorts: the latest GPT baselines and Qwen3.5-4B/9B
Trace2Skill reruns use the current artifact, whereas the formal \method{} runs
and the aligned Qwen rows use an earlier externally supplied SkillOpt artifact.
Some \method{} rows also differ in admission-policy configuration.  We therefore
treat the current frozen main table as a descriptive benchmark comparison rather
than a fully paired ablation; controlled component claims are reserved for
Section~\ref{sec:ablation}, and the table note records the reporting caveats.

\subsection{Main Results}
\label{sec:overall_results}

Table~\ref{tab:main-results} compares final test accuracy across three datasets
and six Action-Agent backbones.  Among the 17 model--dataset cells with a numeric
\method{} result in the current frozen Acc snapshot, \method{} is best or tied
for best in 9 and ranks in the top two in 16.  Relative to NoSkill, it improves
all 17 cells by a cell-macro average of 18.46 percentage points.  The largest
gains occur on ALFWorld with Qwen3.5-4B (+41.79 points) and Qwen3.5-9B
(+36.57 points), followed by ScienceWorld with Qwen3.5-9B (+29.38 points).

\input{experiment/formal_exp}

\subsection{Ablation Study}
\label{sec:ablation}

\input{experiment/ablation}

To answer Q2, we evaluate the full framework against two controlled variants:
\emph{w/o Trigger-Range Replay}, which removes behavior replay from the
Evidence-Grounded Skill Evolution process, and \emph{w/o Cross-Epoch Evidence
Propagation}, which prevents merged Evidence-Linked Edits from being retained
or corrected as Provisional Edits after a rejected full-edit revision.
Table~\ref{tab:ablation} reports eight model--dataset cells spanning two GPT
and two Qwen backbones.  Removing replay lowers accuracy in seven cells, with
AppWorld Qwen3.5-9B as the sole exception.  Removing Cross-Epoch Evidence
Propagation lowers accuracy in five cells and leaves three unchanged; the
ablated variant never outperforms Full.  The largest drops occur on
AppWorld with GPT-5.5
($-8.33$ points without Cross-Epoch Evidence Propagation) and Qwen3.5-4B
($-6.54$ points without replay).

\subsection{Mechanism Analysis}
\label{sec:mechanism_analysis}

To answer Q3, we audit 16 complete formal runs covering 64 skill-evolution
epochs.  We organize the audit around the two mechanisms introduced in
Section~\ref{sec:method}: replay-based edit filtering and cross-epoch Evidence
reuse.  Replay outcomes use \texttt{accept}, \texttt{reflect}, and
\texttt{reject}; policy-level \texttt{defer} is grouped with \texttt{reject}
for edit-level reporting, while the corresponding Evidence Card can remain
active for later reuse.

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{Figure/replay_edit_outcomes.pdf}
  \caption{Replay outcomes at two stages.  The upper row shows Evidence-window
  replay and the lower row shows Post-validation-reject replay.  In each row,
  the left panel reports the initial \texttt{accept}, \texttt{reflect}, and
  \texttt{reject} shares, while the right panel reports \texttt{recovered} and
  \texttt{not retained} outcomes conditional on reflection.  Percentages are
  event-weighted micro-averages; \texttt{reject} includes policy-level
  \texttt{defer}.}
  \label{fig:replay_edit_outcomes}
\end{figure*}

\subsubsection{Evidence-Grounded Skill Evolution}
\label{sec:evidence_grounded_mechanism_analysis}

\paragraph{Replay-based edit filtering.}
Figure~\ref{fig:replay_edit_outcomes} summarizes 1,172 Evidence-window edits
and 128 post-validation-reject edits.  The left panels show the initial
three-way decision, and the right panels make the reflected subset explicit by
separating recovered edits from edits that are not retained.  Across both
stages, most edits are accepted directly and reflection provides a measurable
recovery path.

\subsubsection{Cross-Epoch Evidence Propagation}
\label{sec:cross_epoch_mechanism_analysis}

\paragraph{Post-rejection Provisional retention.}
Rejected revisions are replayed against the same admission policy before their
edits can enter the Provisional ledger.  The figure below reports this pathway
separately from Evidence-window replay because the two stages have different
denominators.

\input{experiment/cross_epoch_retention}
\input{experiment/evidence_lifecycle}

Per-model replay outcomes are tabulated in Appendix~\ref{app:replay_breakdown};
N/A denotes that post-rejection replay was not executable for that cell.
The contrastive correction audit is reported in Appendix~\ref{app:contrastive_rewrite}.

